On the Linguistic Capacity of Real-Time Counter Automata

Counter machines have achieved a newfound relevance to the field of natural language processing (NLP): recent work suggests some strong-performing recurrent neural networks utilize their memory as counters. Thus, one potential way to understand the success of these networks is to revisit the theory of counter computation. Therefore, we study the abilities of real-time counter machines as formal grammars, focusing on formal properties that are relevant for NLP models. We first show that several variants of the counter machine converge to express the same class of formal languages. We also prove that counter languages are closed under complement, union, intersection, and many other common set operations. Next, we show that counter machines cannot evaluate boolean expressions, even though they can weakly validate their syntax. This has implications for the interpretability and evaluation of neural network systems: successfully matching syntactic patterns does not guarantee that counter memory accurately encodes compositional semantics. Finally, we consider whether counter languages are semilinear. This work makes general contributions to the theory of formal languages that are of potential interest for understanding recurrent neural networks.

==> experiments.tex <==
\section{Experiments}

Do some experiments here?

==> lstm.tex <==
% \subsection{LSTM Counter Languages}

% Finally, we compare the general counter machine to a saturated LSTM. At a high level, the difference between these machines is that the general counter machine's behavior is specified as a finite table based on the zeroness of the counters, whereas the saturated LSTM partitions the space of counter values using linear transformations. Clearly, this creates differences in language recognition capabilities, since the method of determining acceptance from a machine state is different for each model. However, even if we ignore the acceptance layer, the same difference in the internal state updates leads to subtle differences in expressive capacity.
% We formalize this by studying the functions expressible by each model, rather than the languages acceptable.
% We construct a language decidable by such a machine but not the saturated LSTM, as well as a language decidable by the saturated LSTM but not this modified counter machine. Thus, while the two formalisms have similar expressive capacities, they are not equivalent.

% % TODO: Just talk about function expressiveness here?

% For a string $x$ and token $\sigma$, let $\num{\sigma}{x}$ denote the number of $\sigma$'s in $x$. Similarly, for tokens $\sigma$ and $\tau$, let $\num{\sigma - \tau}{x}$ denote $\num{\sigma}{x} - \num{\tau}{x}$.

% \begin{theorem} \label{thm:lstm-gcm}
% There exists a function computable by the saturated LSTM but not general counter machine.
% \end{theorem}

% \begin{proof}
% We construct a function computable by a saturated LSTM with $2$ counters and vocabulary $\{a, b, c, d\}$. The function output is the value of $c_2$, and we use the counter $c_1$ as auxiliary memory. At time $t$, $c_1$ computes $\num{a-b}{x_{:t}}$. Define
% \begin{equation}
%     c_2 = \begin{cases}
%         {\times}0 & \textrm{if} \; c_1 < 0 \\
%         {+}1 & \textrm{if} \; x_t = c \; \textrm{and} \; c_1 \geq 0 \\
%         {-}1 & \textrm{if} \; x_t = d \; \textrm{and} \; c_1 \geq 0 \\
%         {+}0 & \textrm{otherwise.}
%     \end{cases}
% \end{equation}
% \end{proof}

% By construction, this language is decidable by a saturated LSTM. However, we claim no general counter machine can compute $c_2$. If a general counter machine could, it would have apply ${\times}0$ when $0 < \num{a-b}{x_{:t}}$ versus when $\num{a-b}{x_{:t}} \leq 0$ to distinguish between the resulting configurations. But this is impossible, since the general counter machine only observes the zeroness of the counters, not their value, and thus cannot implement a $<$ check.

% \begin{theorem}
% There exists a counter function computable by a saturated LSTM but not by a general counter machine.
% \end{theorem}

% \begin{proof}
% We construct a function computable by the general counter machine. Apply the same construction as \autoref{thm:lstm-gcm}, but with the modified $c_2$ update:
% \begin{equation}
%     c_2 = \begin{cases}
%         {\times}0 & \textrm{if} \; c_1 \neq 0 \\
%         {+}1 & \textrm{if} \; x_t = c \; \textrm{and} \; c_1 = 0 \\
%         {-}1 & \textrm{if} \; x_t = d \; \textrm{and} \; c_1 = 0 \\
%         {+}0 & \textrm{otherwise.}
%     \end{cases}
% \end{equation}
% \end{proof}

% By construction, $c_2$ is computable by a general counter machine. A saturated LSTM computing $c_2$ needs to apply ${\times}0$ exactly when $\num{a-b}{x_{:t}} \neq 0$. This corresponds to a set of counter values with two unconnected components: ${<}0$ and ${>}0$. The saturated LSTM implements ${\times}0$ by the coefficient $o_tf_t$, which geometrically corresponds to the intersection of two linearly separable regions, which cannot produce unconnected components. So, the saturated LSTM cannot compute $c_2$.

% % x0 if c_1 \neq 0
% % +1 if x = c
% % -= if x = d
% % +0 otherwise
